The Gaussian Transform

We introduce the Gaussian transform (GT), an optimal transport inspired iterative method for denoising and enhancing latent structures in datasets. Under the hood, GT generates a new distance function (GT distance) on a given dataset by computing the $\ell^2$-Wasserstein distance between certain Gaussian density estimates obtained by localizing the dataset to individual points. Our contribution is twofold: (1) theoretically, we establish firstly that GT is stable under perturbations and secondly that in the continuous case, each point possesses an asymptotically ellipsoidal neighborhood with respect to the GT distance; (2) computationally, we accelerate GT both by identifying a strategy for reducing the number of matrix square root computations inherent to the $\ell^2$-Wasserstein distance between Gaussian measures, and by avoiding redundant computations of GT distances between points via enhanced neighborhood mechanisms. We also observe that GT is both a generalization and a strengthening of the mean shift (MS) method, and it is also a computationally efficient specialization of the recently proposed Wasserstein Transform (WT) method. We perform extensive experimentation comparing their performance in different scenarios.

==> introduction.tex <==
\section{Introduction}
\label{sec:intro}

Optimal Transport (OT) studies how to find an optimal strategy for transporting a source probability measure to a target probability measure \cite{villani2008optimal}. Recently, OT has been widely applied in Machine Learning~\cite{courty2016optimal,peyre2019computational}, Deep Neural Network~\cite{arjovsky2017wasserstein,gulrajani2017improved} and Natural Language Processing 
(NLP)~\cite{alvarez-melis-jaakkola-2018-gromov}, etc.

In \cite{pmlr-v97-memoli19a}, the authors introduced the \emph{Wasserstein transform} (WT) as a method for enhancing and denoising datasets. The WT alters the distance function on a dataset by computing the dissimilarity between neighborhoods of data points via methods from OT. WT can be regarded as a generalization and strengthening of mean shift (MS) \cite{fukunaga1975estimation,cheng1995mean}. Inspired by the construction of WT, in this paper we propose the \emph{Gaussian transform} (GT), a computationally efficient specialization of WT. 


GT takes as input a point cloud and iteratively alters its metric based on how different are the local covariance matrices around points. {This is done via the computation of the $\ell^2$-Wasserstein distance between certain Gaussian distributions associated to these neighborhoods.} See Figure~(\ref{fig:ill-cov}) for an illustration. Due to the fact that there exists a closed form solution for the $\ell^2$-Wasserstein distance between Gaussian distributions
, the computation of GT is substantially more efficient than that of WT (which requires solving an OT problem for \emph{each pair of points} thus having complexity which scales cubically with the size of neighborhoods). 
We show ways of accelerating the computation of GT which include a {novel observation} stemming from computational linear algebra techniques (see Theorem \ref{thm:redux}) and some refinements about neighborhood mechanisms (see Section \ref{sec:nbh-mech}). We also prove that GT is stable with respect to perturbations (cf. Theorem \ref{thm:GT-stable}). 

One important feature of GT is its \emph{sensitivity to anisotropy}, an often desired feature in methods for image denoising and image segmentation 
\cite{perona1990scale,wang2004image}; see Figure \ref{fig:GT}. GT contains an intrinsic parameter $\lambda$ providing flexibility in tuning the degree of sensitivity to anisotropy in data features.
We apply GT to clustering and denoising tasks, and verify that in these, by tuning the parameter $\lambda$, GT has either comparable or superior performance over WT. We further apply GT to image segmentation, a task in which GT outperforms MS \cite{demirovic2019implementation}, and also in NLP tasks to boost word embeddings performance. Our experiments indicate that GT is effective in enhancing and denoising datasets. 
\begin{figure}[htb]
    \centering
    \includegraphics[width=0.9\linewidth]{figures/illustration-gt.pdf}
    \caption{Illustration of GT. 
    We illustrate the idea of GT based on a point cloud in $\R^2$. Different points in the point cloud have different neighborhood structures, which are captured by their local covariance matrices. We  generate a Gaussian distribution \emph{on each data point} based on local covariance matrices. In the figure, we represent these Gaussians by ellipses (iso-contours of Gaussian distributions at a given height). Note that these localized Gaussian distributions reflect the neighborhood structures: the Gaussian is round when the neighborhood is relatively isotropic (\textbf{A} and \textbf{B}); the Gaussian is {flat} when the neighborhood is oblong (\textbf{C, D, E} and \textbf{F}); and the Gaussian is degenerate for an isolated point (cf. \textbf{G}). In a nutshell, the Gaussian Transform produces a new distance function on the dataset by computing the $\ell^2$-Wasserstein distance between these localized Gaussian distributions.
    }
    \label{fig:ill-cov}
\end{figure}

==> preamble.tex <==
%%%our own package
\usepackage{relsize}
\usepackage{amsmath,amscd}
\usepackage{mathtools}
\usepackage{amsthm}
\usepackage{amssymb}
\usepackage{tikz-cd}
\usepackage{color}
\usepackage{bm}
\usepackage{subfig}
\usepackage{caption}
\usepackage{algorithm}
\usepackage{algorithmic}
\usepackage[normalem]{ulem}
\usepackage{graphics}
\usepackage{grffile}

\usepackage{xr}
\makeatletter
\newcommand*{\addFileDependency}[1]{
  \typeout{(#1)}
  \@addtofilelist{#1}
  \IfFileExists{#1}{}{\typeout{No file #1.}}
}
\makeatother

\newcommand*{\myexternaldocument}[1]{
    \externaldocument{#1}
    \addFileDependency{#1.tex}
    \addFileDependency{#1.aux}
}
%%% END HELPER CODE
% \newif\ifdebugdoc\debugdocfalse
\newif\ifdebugdoc\debugdoctrue

\ifdebugdoc

%% Writing Mode
\newcommand{\outline}[1]{\colorbox{yellow}{Outline:}\textcolor{red}{#1}}
\newcommand{\todo}[1]{\large{\colorbox{red}{TODO:} #1. }}
%\newcommand{\fyi}[1]{\footnote{\textcolor{blue}{fyi:#1}}}
%\newcommand{\remind}[1]{\footnote{\textit{[\uwave{Remind:} #1]}}}
\newcommand{\repl}[2]{\textcolor{red}{#1}\textcolor{blue}{\sout{#2}}}
\newcommand{\add}[1]{\textcolor{red}{#1}}
\newcommand{\del}[1]{\textcolor{blue}{\sout{#1}}}
\newcommand{\save}[1]{}
\else
%%Submission Mode
\newcommand{\outline}[1]{}
\newcommand{\todo}[1]{}
\newcommand{\chunyi}[1]{}
\newcommand{\fhl}[1]{#1}
%\newcommand{\fhl}[1]{\textcolor{blue}{{#1}}}
\newcommand{\repl}[2]{#1}
\newcommand{\add}[1]{#1}
\newcommand{\del}[1]{}
\newcommand{\save}[1]{}
\newcommand{\frepl}[2]{\textcolor{red}{#1}\textcolor{blue}{\sout{#2}}}
%\newcommand{\fadd}[1]{\textcolor{red}{#1}}
%\newcommand{\fdel}[1]{\textcolor{blue}{\sout{#1}}}
\newcommand{\fadd}[1]{\textcolor{black}{#1}}
\newcommand{\fdel}[1]{\textcolor{blue}{\sout{#1}}}
\fi

\newcommand{\dis}{\mathrm{dis}}
\newcommand{\diam}{\mathrm{diam}}
\newcommand{\rad}{\mathrm{rad}}
\newcommand{\mean}{\mathrm{mean}}
\newcommand{\tr}{\mathrm{tr}}
\newcommand{\cov}{\mathrm{cov}}
\newcommand{\vol}{\mathrm{vol}}
\newcommand{\supp}{\mathrm{supp}}
\newcommand{\llrrparen}[1]{
  \left(\mkern-6mu\left(#1\right)\mkern-6mu\right)}
  
\newcommand{\bxe}{B_\eps^{d_X}(x)}


\newcommand{\N}{\mathbb{N}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\eps}{\varepsilon}
\newcommand{\bg}{\mathcal{BG}}
\newcommand{\norm}[1]{\left\lVert#1\right\rVert}
\newcommand{\pf}{\mathcal{P}_f}
\newcommand{\wt}[1]{\mathbf{W}_{#1}}
\newcommand{\G}{\mathrm{G}}
\newcommand{\g}{\mathcal{G}}
\newcommand{\gkm}{\g_{k,m-k}}
\newcommand{\vkm}{\mathcal{V}_{k,m}}

\newcommand{\deps}{d_\alpha^{\mathsmaller{(\eps)}}}

\newcommand{\depsbeta}{d_\beta^{\mathsmaller{(\eps)}}}

\newcommand{\lms}{L^{\mathrm{ms}}}



\newcommand{\p}{^\prime}
\newcommand{\pp}{^{\prime\prime}}
\newcommand{\we}[1]{\mathbf{W}_\eps^{#1}}
\newcommand{\me}{m^{\mathsmaller{(\eps)}}}
\newcommand{\de}{d^{\mathsmaller{(\eps)}}}
\newcommand{\lc}{\left(}
\newcommand{\rc}{\right)}
\newcommand{\ls}{\left|}
\newcommand{\rs}{\right|}
\newcommand{\mg}[2]{m^{G,\eps}_{#1}(#2)}
\newcommand{\dcov}{d_{\mathrm{cov}}}
\newcommand{\dgt}{d^{\mathsmaller{(\eps,\lambda)}}_{{\alpha,d_X}}}
\newcommand{\bgt}{B_{\mathrm{GT}}}
\newcommand{\blt}{B_{l2}}
\newcommand{\dw}{d_{\mathrm{W},2}}


%%%%%%%%%%%%%%%%%%%%%%%%%%
\newtheorem{theorem}{Theorem}[section]
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{example}[theorem]{Example}
\newtheorem{claim}{Claim} 
\newtheorem{fact}{Fact}
\newtheorem{exercise}{Exercise}
\newtheorem{question}{Question}
\newtheorem{definition}{Definition}
\newtheorem{conjecture}{Conjecture}
